VELVET: a noVel Ensemble Learning approach to automatically locate VulnErable sTatements

Automatically locating vulnerable statements in source code is crucial to assure software security and alleviate developers' debugging efforts. This becomes even more important in today's software ecosystem, where vulnerable code can flow easily and unwittingly within and across software repositories like GitHub. Across such millions of lines of code, traditional static and dynamic approaches struggle to scale. Although existing machine-learning-based approaches look promising in such a setting, most work detects vulnerable code at a higher granularity -- at the method or file level. Thus, developers still need to inspect a significant amount of code to locate the vulnerable statement(s) that need to be fixed. This paper presents VELVET, a novel ensemble learning approach to locate vulnerable statements. Our model combines graph-based and sequence-based neural networks to successfully capture the local and global context of a program graph and effectively understand code semantics and vulnerable patterns. To study VELVET's effectiveness, we use an off-the-shelf synthetic dataset and a recently published real-world dataset. In the static analysis setting, where vulnerable functions are not detected in advance, VELVET achieves 4.5x better performance than the baseline static analyzers on the real-world data. For the isolated vulnerability localization task, where we assume the vulnerability of a function is known while the specific vulnerable statement is unknown, we compare VELVET with several neural networks that also attend to local and global context of code. VELVET achieves 99.6% and 43.6% top-1 accuracy over synthetic data and real-world data, respectively, outperforming the baseline deep-learning models by 5.3-29.0%.

==> tables/infer_results.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{\small \textbf{
Evaluation of different models on {\sc \textbf{Juliet}} and {\datasetbf} datasets. 
Shown is the localization accuracy and the average distance between the predicted location vs ground truth location.
Best metrics are highlighted in bold red.
}}
%{\sc Juliet:} Min: 4, Max: 202, Mean: 29.57, Median: 20. {\sc Github-Infer:} Min:3, Max: 1844, Mean: 80.05, Median: 46
\label{tab: infer_juliet_acc}
%\normalsize
\small
\begin{tabular}{ll|cc|cccccr}\toprule
\multicolumn{2}{l}{\multirow{3}{*}{Model}} &\multicolumn{2}{l}{JULIET Dataset} &\multicolumn{4}{l}{\dataset Dataset} \\\cmidrule{3-8}
& &\multirow{2}{*}{Localization Acc (\%)} &\multirow{2}{*}{Avg Distance} &\multicolumn{3}{c}{Localization Acc (\%)} &\multirow{2}{*}{Avg Distance} \\\cmidrule{5-7}
& & &(\# lines) &top-1 &top-3 &top-5 &(\# lines) \\\midrule
{\sc Vloggr} (this work) & & 99.1 &{0.01} &\textbf{\textcolor{red}{19.5}} &\textbf{\textcolor{red}{37.9}} &\textbf{\textcolor{red}{48.7}} &\textbf{\textcolor{red}{8.1}} \\\midrule
GGNN & & 96.7 &0.31 &3.6 &6.3 &8.6 &8.9 \\\midrule
RNN & & 99.0 &0.02 &0.4 &2.4 &5.2 &10.1 \\\midrule
Transformer & & 98.1 &0.07 &0.6 &2.4 &4.5 &9.2 \\\midrule
Transformer-sandwich & & 99.1 &{0.01} &12.1 &30.4 &41.6 &8.7 \\\midrule
GREAT & & 98.7 &0.39 &1.3 &3.9 &8.3 &9.9 \\\midrule
Hoppity & & 97.7 &0.15 &8.0 &20.6 &28.3 &8.6 \\\midrule
RNN-sandwich & & \textbf{\textcolor{red}{99.4}} &{0.01} &6.7 &13.5 &19.3 &10.3 \\
% Our Model &Transformer-GGNN++ &99.08\% &0.09 &\textbf{19.51\%} &\textbf{37.96\%} &\textbf{48.74\%} &\textbf{56.61} \\\midrule
% \multirow{3}{*}{Baselines} &GGNN &96.74\% &2.14 &3.62\% &6.31\% &8.56\% &62.77 \\
% &RNN &99.02\% &0.19 &0.38\% &2.39\% &5.20\% &70.65 \\
% &Transformer &98.09\% &0.47 &0.60\% &2.42\% &4.47\% &64.61 \\\midrule
% \multirow{4}{*}{Related Work} &Transformer-sandwich &99.08\% &0.10 &12.06\% &30.42\% &41.59\% &60.67 \\
% &GREAT &98.71\% &0.39 &1.32\% &3.96\% &8.31\% &69.73 \\
% &Hoppity &97.72\% &1.05 &8.01\% &20.58\% &28.29\% &60.07 \\
% &RNN-sandwich &\textbf{99.38\%} &\textbf{0.05} &6.69\% &13.46\% &19.30\% &72.46 \\
\bottomrule
\vspace{-3mm}
\end{tabular}
\end{table*}

==> tables/infer_results_org.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{\small \textbf{Evaluation of different models on both {\sc \textbf{Juliet}} and {\sc \textbf{Github-Infer}}. Localization Acc indicates the accuracy. Avg Distance measures the average prediction distance over all test samples. \ssc{Drop the first column. Treat them as 7 together.}}}
%{\sc Juliet:} Min: 4, Max: 202, Mean: 29.57, Median: 20. {\sc Github-Infer:} Min:3, Max: 1844, Mean: 80.05, Median: 46
\label{tab: infer_juliet_acc}
%\normalsize
\small
\begin{tabular}{ll|cc|cccccr}\toprule
\multicolumn{2}{l}{\multirow{3}{*}{Model}} &\multicolumn{2}{l}{Juliet Dataset} &\multicolumn{4}{l}{Github-Infer Dataset} \\\cmidrule{3-8}
& &\multirow{2}{*}{Localization Acc} &\multirow{2}{*}{Avg Distance} &\multicolumn{3}{c}{Localization Acc} &\multirow{2}{*}{Avg Distance} \\\cmidrule{5-7}
& & &(\# lines) &top-1 &top-3 &top-5 &(\# lines) \\\midrule
Our Model &{\sc Vloggr} &99.08\% &\textbf{0.01} &\textbf{19.51\%} &\textbf{37.96\%} &\textbf{48.74\%} &\textbf{8.09} \\\midrule
\multirow{3}{*}{Baselines} &GGNN &96.74\% &0.31 &3.62\% &6.31\% &8.56\% &8.97 \\
&RNN &99.02\% &0.02 &0.38\% &2.39\% &5.20\% &10.09 \\
&Transformer &98.09\% &0.07 &0.60\% &2.42\% &4.47\% &9.23 \\\midrule
\multirow{4}{*}{Related Work} &Transformer-sandwich &99.08\% &\textbf{0.01} &12.06\% &30.42\% &41.59\% &8.67 \\
&GREAT &98.71\% &0.39 &1.32\% &3.96\% &8.31\% &9.96 \\
&Hoppity &97.72\% &0.15 &8.01\% &20.58\% &28.29\% &8.58 \\
&RNN-sandwich &\textbf{99.38\%} &\textbf{0.01} &6.69\% &13.46\% &19.30\% &10.35 \\
% Our Model &Transformer-GGNN++ &99.08\% &0.09 &\textbf{19.51\%} &\textbf{37.96\%} &\textbf{48.74\%} &\textbf{56.61} \\\midrule
% \multirow{3}{*}{Baselines} &GGNN &96.74\% &2.14 &3.62\% &6.31\% &8.56\% &62.77 \\
% &RNN &99.02\% &0.19 &0.38\% &2.39\% &5.20\% &70.65 \\
% &Transformer &98.09\% &0.47 &0.60\% &2.42\% &4.47\% &64.61 \\\midrule
% \multirow{4}{*}{Related Work} &Transformer-sandwich &99.08\% &0.10 &12.06\% &30.42\% &41.59\% &60.67 \\
% &GREAT &98.71\% &0.39 &1.32\% &3.96\% &8.31\% &69.73 \\
% &Hoppity &97.72\% &1.05 &8.01\% &20.58\% &28.29\% &60.07 \\
% &RNN-sandwich &\textbf{99.38\%} &\textbf{0.05} &6.69\% &13.46\% &19.30\% &72.46 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/juliet_type.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{\small \textbf{
Distribution of vulnerabilities in the datasets.
Columns 1 and 2 show how the vulnerability types in {\datasetbf} map to the corresponding CWEs in \julietbf. Columns 3 and 4 show the respective proportions of the vulnerability type occurrences in the two datasets.
Note that \julietbf covers many more vulnerability types than \datasetbf.
}}
\label{tab:juliet_distribution}
%Distribution of vulnerabilities in the training data. We match the vulnerability types in {\dataset} with the corresponding CWEs in {\sc Juliet}: the first column indicates the type in \dataset; the second column indicates the CWE number that matches the type on the left and exists in {\sc Juliet};  the third column indicates the ratio of such types in the training split of {\sc Juliet}.}}\label{tab:juliet_distribution}
\small
\begin{tabular}{lrcc}\toprule
\textbf{D2A-FUNC} &\textbf{{\sc \textbf{Juliet}}} &\textbf{\sc \textbf{Juliet}}    &\textbf{{\sc \textbf{D2A-FUNC}}} \\ 
\textbf{{\textbf{Category}}} &\textbf{{\textbf{Category}}} &\textbf{Ratio} &\textbf{Ratio} \\
\midrule
\multirow{3}{*}{Buffer Overrun} &CWE121-122 &\multirow{3}{*}{ 25.0\%} &\multirow{3}{*}{ 30.8\%} \\
&CWE124 & \\
&CWE126-127 & \\\midrule
%Dangling Ptr Dereference &unknown &0.0\% &0.3\%\\\midrule
Dead Store &CWE563 &1.0\% &1.3\%\\\midrule
Divide by Zero &CWE369 &1.6\% &0.3\%\\\midrule
\multirow{2}{*}{Integer Overflow} &CWE190-191 &\multirow{2}{*}{21.9\%} &\multirow{2}{*}{56.3\%}\\
&CWE194-197 & \\\midrule
Memory Leak &CWE401 &2.0\% &0.9\%\\\midrule
Null Dereference &CWE690 &1.9\% &3.0\%\\\midrule
NullPtr Dereference &CWE476 &0.7\% &4.9\%\\\midrule
Uninitialized Value &CWE457 &1.6\% &1.9\%\\\midrule
Use After Free &CWE416 &0.4\% &0.04\%\\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table}

==> tables/juliet_varied_graph.tex <==
%Please add the following packages if necessary:
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{\small \textbf{Vulnerability localization performance of different code graphs on \julietbf dataset. %Localization Acc indicates the accuracy. 
Avg Distance measures the average prediction distance over all test samples.}}
\small
\begin{tabular}{cccr}\toprule
Graph  &Localization  &Avg Distance  \\
 Structure &Accuracy & (\# lines) \\ \midrule
CPG &\textbf{96.74} &0.31 \\\midrule
AST &93.73 &0.40  \\\midrule
CFG &93.73 &0.51 \\\midrule
DFG &92.17 &0.53 \\\midrule
AST + CFG &95.94 &0.36 \\\midrule
AST + DFG &95.14 &\textbf{0.24} \\\midrule
CFG + DFG &94.03 &0.49 \\\midrule
AST+CFG+DFG &95.82 &0.29 \\
% CPG &\textbf{96.74} &2.14 \\\midrule
% AST &93.73 &2.80 \\\midrule
% CFG &93.73 &3.54 \\\midrule
% DFG &92.17 &3.70 \\\midrule
% AST + CFG &95.94 &2.49 \\\midrule
% AST + DFG &95.14 &\textbf{1.70} \\\midrule
% CFG + DFG &94.03 &3.42 \\\midrule
% AST+CFG+DFG &95.82 &2.03 \\
\bottomrule
\end{tabular}
\label{tab: juliet_varied_graph}
\end{table}

==> tables/rq1_prec_rec_f1.tex <==
\begin{table}[h]\centering
\vspace{-2mm}
\caption{\small Results of Precision, Recall and F1 metrics for function-level vulerability detection.}\label{tab: precision_recall_f1}
\scriptsize
\begin{tabular}{lrrrrrrr}\toprule
\multirow{2}{*}{Approach} &\multicolumn{3}{c}{\juliet} &\multicolumn{3}{c}{\dataset} \\\cmidrule{2-7}
&Precision &Recall &F1 &Precision &Recall &F1 \\\midrule
\tool & & & & & & \\
Ensemble &\textbf{99.9\%} &\textbf{99.3\%} &\textbf{99.6\%} &\textbf{76.2\%} &48.1\% &\textbf{59.0\%} \\
GGNN &\textbf{99.9\%} &89.0\% &94.2\% &73.2\% &39.1\%  &51.0\% \\
Transformer &\textbf{99.9\%} &\textbf{99.3\%} &\textbf{99.6\%} &70.5\% &\textbf{50.4}\% &58.8\% \\
\midrule
Infer &41.5\% &54.4\% &47.1\% &N/A &N/A &N/A \\
FlawFinder &36.6\% &51.0\% &42.6\% &53.3\% & 6.0\% &10.7\% \\
RATS &36.5\% &46.4\% &40.9\% &47.9\% &16.4\% &24.4\% \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table}


==> tables/rq1_results_per_type.tex <==
\begin{table}[!htp]\centering
\caption{This may go to Appendix}\label{tab: rq_1_type_result}
\scriptsize
\begin{tabular}{lrrrrrrr}\toprule
\multirow{2}{*}{Model} &Integer &Buffer &NullPointer &Dead &Memory &Dangling Pointer \\
&Overflow &Overrun &Dereference &Store &Leak &Dereference \\\midrule
{\sc Vloggr-ensemble} &45.5\% &45.8\% &20.0\% &0.0\% &0.0\% &0.0\% \\
{\sc Vloggr-ggnn} &36.4\% &33.3\% &20.0\% &0.0\% &0.0\% &0.0\% \\
{\sc Vloggr-trans} &40.3\% &43.8\% &20.0\% &0.0\% &0.0\% &0.0\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/rq2_results.tex <==
%\vspace{-5mm}
\begin{table}[!htp]\centering
\caption{\small Test performance when jointly training models on vulnerable and non-vulnerable functions. Pred ACC indicates the \emph{Prediction Accuracy} (Section \ref{subsec: rq2}). Vul-CLS ACC indicates the \emph{Vulnerability Detection Accuracy} (Section \ref{subsec: rq2}). Vul-LOC ACC indicates the top-1 localization accuracy (Section \ref{subsec: rq1})}\label{tab: rq2_result}
\scriptsize
\begin{tabular}{lrrrrrrr}\toprule
\multirow{3}{*}{Approach} &\multicolumn{3}{c}{\juliet} &\multicolumn{3}{c}{\dataset} \\\cmidrule(lr){2-4} \cmidrule(lr){5-7}
&Pred &Vul-CLS &Vul-LOC &Pred &Vul-CLS &Vul-LOC \\
&ACC &ACC &ACC &ACC &ACC &ACC \\\midrule
{\sc Velvet} & & & & & & \\
Ensemble &\textbf{\textcolor{red}{99.5\%}} &\textbf{\textcolor{red}{99.6\%}} &\textbf{\textcolor{red}{99.6\%}} &\textbf{\textcolor{red}{51.1\%}} &58.9\% &\textbf{\textcolor{red}{30.1\%}} \\
GGNN &93.6\% &94.2\% &98.5\% &45.5\% &56.7\% &19.6\% \\
Transformer &99.3\% &\textbf{\textcolor{red}{99.6\%}} &99.1\% &47.2\% &\textbf{\textcolor{red}{59.3\%}} &29.3\% \\\midrule
Infer* &N/A &69.4\% &36.9\% &N/A &N/A 
&N/A \\
FlawFinder &N/A &58.3\% &8.6\% &N/A &48.7\% 
&6.7\% \\
RATS &N/A &59.3\% &N/A &N/A &45.8\% &N/A \\
\bottomrule
\end{tabular} \\
\begin{flushleft}
\scriptsize 
*We do not compare with Infer on \dataset, since Zheng \etal~\cite{D2A} used Infer during data collection. Thus, it is unfair to compare with Infer on \dataset. 
%See Section~\ref{sec:threats} for further discussions.
\end{flushleft}

\vspace{-5mm}
\end{table}

==> tables/rq4_result_b.tex <==
\begin{table}[!htp]\centering
\caption{\small \textbf{Vulnerability localization performance of different code graphs on \julietbf dataset. %Localization Acc indicates the accuracy. 
Avg Distance measures the average prediction distance over all test samples.}}
\footnotesize
\begin{tabular}{lccr}\toprule
Graph Structure &Localization Accuracy &Distance \\ \midrule
CPG &\textbf{98.1\%} &\textbf{0.10} \\%\midrule
AST &96.3\% &0.27  \\%\midrule
CFG &96.6\% &0.24 \\%\midrule
DFG &96.5\% &0.33 \\%\midrule
AST + CFG &97.5\% &0.14 \\%\midrule
AST + DFG &96.4\% &0.30 \\%\midrule
CFG + DFG &97.6\% &0.18 \\%\midrule
AST+CFG+DFG &97.4\% &0.14 \\
\bottomrule
\end{tabular}
\label{tab: juliet_varied_graph}
\end{table}

==> tables/vul_type_result.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{\small \textbf{Top-1 localization accuracy for each vulnerability type in \datasetbf. Best stats highlighted in bold red.}}
\label{tab:type_results}
\small
\begin{tabular}{lrrrrrrrrr}\toprule
&\tool &GGNN &RNN &Transformer &Trans-sandwich &GREAT &Hoppity &RNN-sandwich \\\midrule
Buffer Overrun &\textbf{\textcolor{red}{31.1\%}} &5.3\% &0.7\% &0.8\% &18.6\% &1.8\% &12.2\% &10.4\% \\\midrule
Dangling Pointer Dereference &\textbf{\textcolor{red}{25.0\%}} &0.0\% &0.0\% &0.0\% &0.0\% &12.5\% &12.5\% &12.5\% \\\midrule
Dead Store &0.0\% &0.0\% &0.0\% &0.0\% &0.0\% &0.0\% &\textbf{\textcolor{red}{6.7\%}} &0.0\% \\\midrule
Divide by Zero &\textbf{\textcolor{red}{42.9\%}} &0.0\% &0.0\% &0.0\% &14.3\% &0.0\% &0.0\% &14.3\% \\\midrule
Integer Overflow &\textbf{\textcolor{red}{13.5\%}} &3.1\% &0.4\% &0.6\% &8.5\% &1.3\% &5.7\% &4.4\% \\\midrule
Memory Leak &0.0\% &0.0\% &0.0\% &0.0\% &\textbf{\textcolor{red}{5.0\%}} &0.0\% &\textbf{\textcolor{red}{5.0\%}} &\textbf{\textcolor{red}{5.0\%}} \\\midrule
Null Dereference &\textbf{\textcolor{red}{12.7\%}} &4.2\% &1.4\% &0.0\% &11.3\% &0.0\% &5.6\% &7.0\% \\\midrule
NullPtr Dereference &\textbf{\textcolor{red}{25.6\%}} &1.7\% &0.0\% &0.0\% &13.7\% &0.0\% &8.6\% &2.6\% \\\midrule
Uninitialized Value &\textbf{\textcolor{red}{21.7\%}} &2.2\% &0.0\% &0.0\% &19.6\% &0.0\% &13.0\% &10.9\% \\\midrule
Use After Free &\textbf{\textcolor{red}{100.0\%}} &0.0\% &0.0\% &0.0\% &\textbf{\textcolor{red}{100.0\%}} &0.0\% &\textbf{\textcolor{red}{100.0\%}} &0.0\% \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table*}
